The Vulnerable Nature of Decentralized Governance in DeFi

Decentralized Finance (DeFi) platforms are often governed by Decentralized Autonomous Organizations (DAOs) which are implemented via governance protocols. Governance tokens are distributed to users of the platform, granting them voting rights in the platform's governance protocol. Many DeFi platforms have already been subject to attacks resulting in the loss of millions of dollars in user funds. In this paper we show that governance tokens are often not used as intended and may be harmful to the security of DeFi platforms. We show that (1) users often do not use governance tokens to vote, (2) that voting rates are negatively correlated to gas prices, (3) voting is very centralized. We explore vulnerabilities in the design of DeFi platform's governance protocols and analyze different governance attacks, focusing on the transferable nature of voting rights via governance tokens. Following the movement and holdings of governance tokens, we show they are often used to perform a single action and then sold off. We present evidence of DeFi platforms using other platforms' governance protocols to promote their own agenda at the expense of the host platform.

==> README <==
This package provides a class for typesetting publications of the
Association for Computing Machinery.

Your TeX distribution probably includes the latest released version of
this package.  If you decide to install it yourself, please see the
Installation section of the User's Guide.

Please note that the version on Github is a development (or
experimental) version: please download it for testing new features.
The production version is the one on CTAN and ACM sites.


Changes

Version 1.90   Journal ISSN updated

Version 1.89a  Added version info to .bst

Version 1.89   Bug fixes
	       Redesign of ACMCP
	       New positioning of badges
	       New journals: PACMMOD, TOPML

Version 1.88   New ISSNs
	       Documentation updates
	       New journal:  PACMNET

Version 1.87   CC license is allowed for non-acm documents and ACM Engage
	       documents only
	       New format acmcp for the cover page
	       New journals: JATS, ACMJCSS, TORS
	       Bug fixes

Version 1.86.  Empty country in affiliation now produces an error
               Bug fixes
	       New samples for acmengage

Version 1.85.  Bug fixes
	       Added support for Creative Commons licenses (requires
	       doclicense images)
	       New journals
	       New format acmengage for ACM Engage CSEdu course materials 

Version 1.84   Support for BibLaTeX rewritten (thanks to
	       Roberto Di Cosmo and Kartik Singhal)
	       Corrected German translation (thanks to Dirk Beyer)
	       New journals

Version 1.83   Support for multilanguage papers
	       ISSN changes for some journals

Version 1.82   Bug fixes.
	       New command \anon for anonymization of short strings.
	       Documentation update.

Version 1.81   Bug fixes
	       New bib field distinctURL to print URL even if doi is present.
	       Reworded samples

Version 1.80   New journals: DLT, FAC

Version 1.79   Fixed pages with index
	       (https://github.com/borisveytsman/acmart/issues/440)
	       Updated information for TAP, TCPS, TEAC

Version 1.78   Documentation update.
	       Magic texcount comments for samples.
	       Title page now is split if there are too many authors
	       Bug fixes.

Version 1.77   Changed the way to typeset multiple affiliations (Christoph Sommer)

Version 1.76   Added many journal abbreviations to the bst.
	       New experimental option: pbalance
	       ORCID linking code

Version 1.75   Omitted \country now produces error.
	       Added \AtBeginMaketitle

Version 1.74   Bug fixes.  A regression introduced in the font changes
	       is reverted.

Version 1.73   Bug fixes
	       The elements institution, city and country are now obligatory
	       for affiliations.  The absence of them produces a warning

Version 1.72   Bug fixes.  Better handling of metadata.

Version 1.71   Bug fixes
               Formats sigchi and sigchi-a are retired
	       Bibliography formatting changes for @inproceedings entries
	       having both series and volume
	       LuaLaTeX now uses the same OTF fonts as XeLaTeX

Version 1.70   Title change for ACM/IMS Transactions on Data Science
               Bug fixes for bibliography

Version 1.69   Bug fixes
	       Compatibility with LaTeX 2020-02-02 release

Version 1.68   Bug fixes
               BST now recognizes words `Paper' or 'Article' in
	       eid or articleno

Version 1.67   Urgent bug fixes:
	       BibTeX style bug fixed (Michael D. Adams)
	       Sigplan special section bugfix

Version 1.66   Bug fixes
	       BibTeX change:  location is now a synonym for city (Feras Saad) 
	       ACM reference format is now mandatory for papers over one page.
	       CCS concepts and keywords are now mandatory for
	       papers over two pages.
	       Authors' addresses are mandatory for journal articles.

Version 1.65   Bug fixes
	       New journal: DGOV
	       DTRAP and HEALTH are now using acmlarge format

Version 1.64    Produce error if abstract is entered after maketitle
		(previously abstract was silently dropped)
		Bug fixes for line numbering

Version 1.63a   Moved TQUANT to TQC

Version 1.63	New journals: TQUANT, FACMP

Version 1.62    Documentation update
		New journal: TELO
		Bug fixes

Version 1.61    Bug fixes
                New bibtex types for artifacts

Version 1.60    New option: urlbreakonhyphens (thanks to Peter Kemp)
		Smaller header size for acmsmall

Version 1.59    Now a journal format can be used for conference proceedings
		All samples are now generated from the same .dtx file
		Bug fixes

Version 1.58    Suppressed spurious warnings.
		New journal:  HEALTH.
		TDSCI is renamed to TDS.

Version 1.57    Change of \baselinestretch now produces an error
                Booktabs is now always loaded
                Added option `balance' to balance last page in two-column mode
                E-mail is no longer split in addresses
                New samples (Stephen Spencer)

Version 1.56    Bug fixes
                Added \flushbottom to two column formats (Philip Quinn)
                The final punctuation for the list of concepts
                is now a period instead of a semicolon (Philip Quinn)
                New command \Description to describe images for visually
                impaired users.

Version 1.55    Bug fixes
                Font changes for SIGCHI table captions

Version 1.54    New option: 'nonacm' (Gabriel Scherer)
                Deleted indent for subsubsection (suggested by Ross Moore)
                Suppressed some obscurious warning in BibTeX processing
                Suppressed hyperrerf warnings (Paolo G. Giarrusso)
                New code for sections to help with accessibility patches
                (Ross Moore)
                Submission id, if present, is printed in anon mode
                Bug fixes

Version 1.53    New journals: PACMCGIT, TIOT, TDSCI

Version 1.52    Another rewording of licenses

Version 1.51    Journal footers now use abbreviated journal titles.
                Corrected the bug with acmPrice.
                Do not show price when copyright is set to iw3c2w3 and iw3c2w3g.
                The package now is compatible with polyglossia (Joachim Breitner).
                Slightly reworded copyright statements.

Version 1.50    Changes in iw3c2w3 and iw3c2w3g

Version 1.49    New jorunal:  DTRAP

Version 1.48    Bug fixes
                Review mode now switches on folios
                Code prettying (Michael D. Adams)
                Bibliography changes: @MISC entries no longer have a
                separate date
                Sigch-a sample bibliography renamed
                Bib code cleanup (Zack Weinberg)
                Acmart and version info are added to pdfcreator tag
                \citeyear no longer produces parenthetical year
                Added initial support for Biblatex (Daniel Thomas)
                Added support for IW3C2 conferences

Version 1.47    New journal: THRI

Version 1.46    Bug fixes for bibliography: label width is now calculated
                correctly.
                All PACM now use screen option.  This requires etoolbox.
                Added subtitle to ACM reference format.
                Now acmart is compatible with fontspec.
                \thanks is now obsolete.  The addresses are automatically
                added to the journal version; this can be overriden with
                \authorsaddresses command.
                Deleted the rule at the end of frontmatter for all formats.
                Deleted new line before doi in the reference format.
                Reintegrated theorem code into acmart.dtx (Matthew Fluet)

Version 1.45    Workaround for a Libertine bug.  Thanks to LianTze Lim
                from Overleaf

Version 1.44    Bug fixes.
                Empty DOI and ISBN suppress printing DOI or ISBN lines
                Separated theorem code into acmthm.sty, loaded by default.
                Article number can be set for proceedings.
                New commands: \acmBooktile, \editor.
                Reference citation format updated.

Version 1.43    Bug fixes

Version 1.42    Deleted ACM badges
                Bug fixes

Version 1.41    Rearranged bib files
                Added new badges

Version 1.40    Bibliography changes
                Added processing of one-compoment ccsdesc nodes
                Bug fixes.
                Made the height a multiple of \baselineskip + \topskip
                Added cleveref
                We no longer print street address in SIGs

Version 1.39    Added \authornotemark commmand

Version 1.38    Increase default font size for SIGPLAN

Version 1.37    Reduce list indentation (Matthew Fluet)

Version 1.36    Bug fixes
                Moved PACMPL to acmlarge format
                New journal: PACMHCI
                Added the possibility to adjust number of author
                boxes per row in conference formats

Version 1.35    Author-year bib style now uses square brackets.
                Changed defaults for TOG sample
                Price is suppressed for usgov and rightsretained modes.
                Bugs fixed

Version 1.34    Deleted DOI from doi numbers
                Changed bibstrip formatting
                The command \terms is now obsolete
                The rulers in review mode now have continuous numbering

Version 1.33    New option `timestamp' (Michael D. Adams)
                New option `authordraft'
                Documentation updates
                Bug fixes
                We now use Type 1 versions of Libertine fonts even with XeTeX.
                New hook acmart-preload-hook.tex (wizards only!)
                Added new options `obeypunctuation' for \affiliation command
                Added SubmissionID
                Added right line count ruler for two-column formats
                Added workaround for Adobe Acrobat bugs in selection
                Added eid field to the bibliography

Version 1.32    New DOI formatting.
                Format siggraph is now obsolete, and sigconf
                is used instead.
                New proceedings title: POMACS.

Version 1.31    Changed default year and month to the current ones
                (thanks to Matteo Riondato)
                Table of contents now works
                Marginalia now work in all formats
                New command \additionalaffiliation
                Documentation changes

Version 1.30    Bibtex style now recognizes https:// in doi.
                Added \frenchspacing.
                \department now has an optional hierarchy level.
                Switched to T1 encoding
                Updated IMWUT and PACMPL

Version 1.29    Documentation changes.  Head height increased from 12pt to 13pt.
                Removed spurious indent at start of abstract.
                Improved kerning in CCS description list.

Version 1.28    Bug fixes: natbib=false now behaves correctly.

Version 1.27    Bug fixes

Version 1.26    Bug fixes

Version 1.25    Updated PACMPL journal option.

Version 1.24    Added IMWUT journal option.

Version 1.23    Added PACM PL journal option.

Version 1.22    Bibliography changes for Aptara backend; should be
                invisible for the users.

Version 1.21    Bibliography changes: added arXiv, some cleanup

Version 1.20    Bug fixes, documentation updates

Version 1.19    Include 'Abstract', 'Acknowledgements', and 'References'
                in PDF bookmarks.

Version 1.18    Natbib is now the default for all versions.  A unified bib
                file is used for all styles.  Better treatment
                of multiple affiliations.


Version 1.17    Formatting changes for margins and lists.  Bug fixes.

Version 1.16    Formatting changes for headers and footers.

Version 1.15    New structured affiliation command.
                New commands for acknowledgements.

Version 1.14    Warn about undefined citation styles; move definitions
                of acmauthoryear and acmnumeric citation styles before
                use.

Version 1.13    Formatting changes: headers, folios etc.
                Bibliography changes.

Version 1.12    Bug fixes and documentation updates.
                Footnotes rearranged.
                Option natbib is now mostly superfluous: the class
                makes a guess based on the format chosen.

Version 1.11    Customization of ACM theorem styles and proof
                environment (Matthew Fluet).

Version 1.10    Bug fixes

Version 1.09    SIGPLAN: revert caption rules (Matthew Fluet)

Version 1.08    SIGPLAN reformatting (Matthew Fluet); bug fixes


==> governance_protocol_details.tex <==
\section{Key Governance Protocols}\label{app:governance_protocols}
In this section we detail the design of three prominent governance protocols. We focus on safeguards set in place, voting and proposing thresholds and the dependencies between the smart contracts.

\subsection{Aave's Governance Protocol Flow}\label{section:Aave_Governance} 
AAVE (and stkAAVE) token holders receive governance powers proportionally to the sum of their balance.
Token holders are granted two types of power: Proposing and voting. These powers can also be delegated by a token holder to others.
Proposals are divided into two types - short and long.
Short time lock proposals can only affect protocol parameters.
Long time lock proposals can affect governance consensus. These therefore have a longer voting time. They also require a higher voting rate for the proposal.
To introduce a new proposal, a user needs to have a token balance higher than a certain predetermined threshold. This balance is first checked at the block before the proposal is created and needs to remain until the proposal is executed.

The proposing (and voting) power of a user at a given block is computed by taking a snapshot of that account's AAVE/stkAAVE balances plus the balances of all delegators who delegated their tokens to this user.
A users' voting power is calculated when submitVote() is called. 

Aave requires that the life-cycle of a proposal begin off-chain with an Aave Request for Comments (ARCs). Then an Aave Improvement Proposal (AIP) can  be created and submitted by any community member who has sufficient proposition power. The proposal is then parsed and uploaded to IPFS. The returned IPFS hash is used in the following steps in creating the onchain proposal.

A proposal is created with a voting delay. After the voting delay ends, users can start voting on proposals. 
Users can vote for or against the proposal within the duration of the voting period.
Two criteria must be met for a proposal to pass: 
The voting power of for-votes needs exceed a minimum parameter, and The difference between supporting  and  objecting votes needs to exceed a threshold.

Proposals can be cancelled before being executed by the guardian account - A safeguard to the protocol. This account is controlled by a community multisig.

A proposal is created using the create() method in the AaveGovernanceV2 contract~\cite{aave2020AaveGovernanceV2}(0xE.252c) contract. The sane contract is used for voting using the vote() method. Both the total and a specific users' Proposing an voting power can be fetched by calling the  \hyperlink{https://github.com/aave/governance-v2/blob/f7761d9ee6347a3996bea665103d8e2080d8b9b2/contracts/governance/GovernanceStrategy.sol}{AaveGovernanceStrategy} contract. Proposals are executed via executor contracts (\hyperlink{https://etherscan.io/address/0x79426A1c24B2978D90d7A5070a46C65B07bC4299}{long} or \hyperlink{https://etherscan.io/address/0xee56e2b3d491590b5b31738cc34d5232f378a8d5}{short}).

\subsubsection{Voting in Aave}
% \paragraph{Version 1}
% In Aave V1 governance token holders can vote once a proposal enters the ``Voting'' phase. The voting remains open until the end of the voting duration, dictated by the \_votingBlocksDuration. USers can vote  by sending vote transactions using the ``submitVoteByVoter()'' method on the ``AaveProtoGovernance'' (\href{https://etherscan.io/address/0x8a2efd9a790199f4c94c6effe210fce0b4724f52#code}{0x8...f52}) contract.
% A user its vote by re-calling submitVoteByVoter() with the new vote, or alternatively cancel the vote with cancelVoteByVoter() and re-submitting.
% A user can also vote indirectly by submitting a vote by relayer.
% In this protocol, a user may use its tokens to vote, and then sell them off to another user, who may the also use the same tokens to vote. This is known as a ``double voting attack''. To prevent this, Aave V1 realized the function ``challengeVoters()'' on the ``AaveProtoGovernance'' contract. This function can be called by any user to challenge and cancel invalid votes during the time that voting is active. A vote is invalid when the voter's current balance of the voting asset is less than the balance of the same asset at the time of casting their vote, meaning that they have used their tokens for something else after voting (e.g. selling them to someone who wants to double-vote). Note that this means that a user may double-vote with the same tokens many times and get away with it unless someone else actively catches them and cancels the vote. 

% \paragraph{Version 2}
In Aave V2, governance token holders can vote either directly, or by delegating their tokens to another user\\smart contract to vote on their behalf. Voting is done by calling the ``submiteVote()'' function on the ``AaveGovernanceV2'' (\href{https://etherscan.io/address/0xEC568fffba86c094cf06b22134B23074DFE2252c}{0xE...52c}) contract. Delegating voting power is done by calling the ``delegateByType()'' function on the ``AAVE'' (\href{https://etherscan.io/address/0x7fc66500c84a76ad7e9c93437bfc5ac33e2ddae9}{0x7...aE9}) token contract.
Once a proposal turn to the state ACTIVE, users can submit a vote. Users can vote for or against the proposal. The voting power is calculates by counting the users' tokens $+$ delegated voting power, weighed by the total voting power available. This amount is calculated at the same block that the voting turns active, and a user can vote at any time that voting is still active (during the VOTING\_DURATION). Since the voting power is calculated when the voting begins, a user may vote and then use the tokens elsewhere. Even if someone else acquires the same tokens, they will not be able to use them to vote on the same proposal again, since voting power is calculated per user at the beginning of the vote and the buyer did not have possession of these tokens at that time.


\subsubsection{On \& Off Chain Integration}\label{section:offChain}
In Aave's governance suggestion flow, to submit a governance change proposal, one must go through both an off-chain and an on-chain process. We now map several possible failure points in this process and how Aave addresses them. The off-chain process consists largely of two parts. The first is a suggestion phase on Aave's governance forum, called and ``Aave Request for Comments'' (ARC). The next phase is preparing the ``Aave Improvement Proposal'' (AIP), merging it into Aave's repository on Github and uploading it to Aave's IPFS \cite{aaveaips2022aave}. Merging into Aave's code-base is currently controlled by the Aave Genesis Team. Notice that this introduces a a centralization point into Aave's proposal flow - in order for a proposal to be viable, it needs to be merged by a member of Aave's team. Upon uploading the proposal to IPFS, a hash of the upload is created (called the IPFSHash in Aave's smart contract). Aave states that this hash is needed to submit the proposal on-chain in the following phase. This is the phase in the pipeline where The off-chain and on-chain phases should meet and be compared to each other.
In reality, the IPFSHash is never verified on-chain. It is not surprising that the IPFSHash is not verified, as the Ethereum blockchain is an enclosed system with no natural integration currently available for retrieving updated information from outside sources such as IPFS.  This means that a user with sufficient governance tokens can bypass the entire off-chain phase and simply submit a proposal on-chain using the create() method, without consulting the community or Aave's team. It also seems that the only safeguard that Aave has in place for this attack scenario is the ``Guardian'' power. The guardian is a special account that has the power to cancel active proposals without consulting the community, essentially cancelling the votes of governance token holders. This essentially makes the Guardian a dictator in the governance protocol. To summarize this discussion, we see two major points of centralization in the Aave governance flow - The first is Aave's core teams' control over merging into their code-base, and the second is the Guardian dictator currently controlled by Aave's core team. In addition, we see an overwhelming security flaw in Aave's governance design, since anyone can bypass the off-chain part of the protocol, and can only be caught by monitoring the blockchain by Aave's team and cancelled via dictator censorship. 
% \begin{figure}
%     \centering
%     \includegraphics[width=\columnwidth]{AaveGovernancePipeline}
%     \caption{Aave's governance proposal pipeline.}
%     \label{fig:AaveGovernancePipeline}
% \end{figure}

% \subsection{Automatic Proposal Code Validation}
% \todo{Add seatbelt?}

\subsection{Compound's Governance Protocol Flow} 
\label{section:compoundGovernance}


In Compound, A single proposal can include up to 10 actions. Proposals have waiting periods to allow people to vote, and after a proposal is accepted there is an additional waiting period until executing it. A user can only propose a change if he owns  more than 1\% of governance tokens. A proposals can be deleted if you fall below the threshold. This (and the waiting period for voting and execution) prevents flash-loan attacks, or attacks that entail making a lot of proposals just to force people to vote for them and waste funds on gas. Proposals are put in a queue, but one can vote on proposals without accounting for their order.

Currently, the admin for the cUSDT contract is address \href{https://etherscan.io/address/0x6d903f6003cca6255d85cca4d3b5e5146dc33925}{0x6d...925}, which is a \emph{Timelock} smart contract. This contract enables its own admin to queue operations on controlled contracts, which execute after a hard-coded delay of two days. The admin for this contract is another smart contract which is deployed at address 
\href{https://etherscan.io/address/0xc0Da02939E1441F497fd74F78cE7Decb17B66529}{0xc...529} and which delegates function calls to the \emph{GovernanceBravoDelegate} contract deployed at address 
\href{https://etherscan.io/address/0x30065b703de5d473975a2db5bbb790a23fd6efbd}{0x3...fbd}. This contract allows users to propose and vote on actions, according to Compound's governance protocol. The GovernanceBravoDelegate has an admin too, but it is associated with address $0x00\ldots 000$. This address is referred to as the \emph{null} address, the secret key of which is currently widely believed to not be known by anyone \cite{zhao2021temporal}.

\subsection{Uniswaps' Governance Protocol Flow} \label{section:Uniswap_Governance}
Uniswap's governance proposal flow works as follows. It starts off with an extensive off-chain phase: A user should (1) Submit a forum post to Uniswap's governance forum. (2) Use Uniswap's Discord to discuss your proposal in a community call ( which requires interacting with the Discords' admins) and on Twitter Space as well. (3) Create another forum post in the Temperature Check section and publish a snapshot \cite{snapshot2022uniswap} with 2-5 days voting time. This action requires at least 1K UNI tokens delegated or self-delegated. For the snapshot to be valid, at least 25k UNI should participate. (4) A user should then update the temperature check post with the community feedback. (5) Publish a snapshot \href{https://gov.uniswap.org/c/consensus-check/10}{consensus check}. This action requires at least 1K UNI tokens delegated or self-delegated. The snapshot would be deemed valid if at least 50K UNI participates. The \href{fish.vote}{fish.vote} app allows small users to pools their votes to reach the minimum requirements to submit a vote.

Only once these steps have been completes should a user then create an on-chain proposal. The Uniswap governance protocol is made up of three components; the UNI token contract, governance module, made up of the GovernorBravoDelegator contract \href{https://etherscan.io/address/0x408ED6354d4973f66138C91495F2f2FCbd8724C3#code}{0x4$\ldots$ 4C3} which is the address of the proxy governance contract and the GovernorBravoDelegatecontract which is the current implementation address of the governance contract (today this contract is located at \href{https://etherscan.io/address/0x53a328f4086d7c0f1fa19e594c9b842125263026#code}{0x5$\ldots$026} and the , and Timelock. Any addresses with more than 2.5M UNI delegated to it may propose governance changes. An active proposal remains open for voting by the community for $3$ days. A proposal is approved if at least $4$M votes are cast for the proposal, and a majority of the voters supported the proposal. If a proposal is approved, it is  for at least two days in the Timelock contract before being executed.  
The Uniswap governance protocol code is a fork of Compounds' governance protocol code on Github, located at \href{https://github.com/compound-finance/compound-protocol/tree/v2.8.1}{compound-protocol/tree/v2.8.1}. As in Compounds' protocol, there exists a similar ``Guardian'' entity in uniswap which can cancel any proposal that has not yet been executed. 
Voting in Uniswap is done by calling either the ``castVote'' method or the ``castVoteBySig'' method (which allows voting via delegates. The voting power is computed at the time a vote becomes active (as in Compound and Aave V2). See~\cref{fig:compoundGovContract} for a simplified example of the flow of the governance protocol in Compounds' USDT liquidity pool.

\begin{figure}
    \centering
    \includegraphics[width=\columnwidth]{DeFi_governance}
    \caption{Simplified view of Compounds' USDT liquidity pool governance protocol}
    \label{fig:compoundGovContract}
\end{figure}


% \section{Escrowed Governance Tokens}
% \emph{Vote Escrowed Tokenomics} is a different way of issuing governance power to users. It is different from the governance tokens described above (which are minted by the platform and given as rewards for participation. 
% Vote Escrow is a mechanism in which users lock tokens in the platform. In return for locking coins, users are rewarded veTokens, which allow users to vote on the platforms governance. Tokens are distributed according to the time a user committed to locking the funds on the platform. The intuition behind this type of mechanism is that users that believe in the platform should be willing to lock funds for longer time periods, and will therefore make better governance decisions that will benefit the platform. Several DeFi platforms now use veTokens in their governance protocol, including Curve.fi \cite{curve2022veTokens}, Balancer \cite{balancer2022veTokens} and Cream finance. In Curve.fi the $veCRV$ token is controlled by the VotingEscrow contract\cite{curve2022veTokens}, deployed to the Ethereum mainnet at $0x5\ldots A2$. In Curve.fi's system, 
% veCRVs cannot be transferred, they can only be obtained through locking CRV in the platform. 
% \newline
% \newline
% See~\cref{app:governance_protocols} for a thorough overview of the design of the governance protocols of the Aave, Compound and Uniswap platforms. 



==> proxy_design_pattern.tex <==

\section{Governance Protocols via Proxy Design Pattern}\label{app:proxy_design_pattern}
% \subsection{Immutability of Smart Contracts}

Under standard security assumptions (such as a honest mining majority~\cite{eyal2014majority,sompolinsky2016bitcoins}), blockchain transactions are irrevocable. Under Ethereum's EVM, this is extended to deployed smart contract code -- once a contract is deployed to the blockchain, transactions cannot modify its code other than outright erasing it~\cite{wood2014ethereum}. E.g., smart contract are \emph{immutable}.
This might lead an unsuspecting user to believe that a DeFi platform that is run algorithmically will never change, e.g., that bugs or design flaws cannot be easily corrected. In particular, the notion that code cannot be change contradicts the premise of governance protocols, which should allow users to propose and vote on changes to the logic which underlies smart contracts.

To circumvent this limitation, various platforms utilize the so-called \textit{Proxy Design Pattern}~\cite{marchesi2020design}, which allows modifying contracts after deployment by employing a multi-contract design in which calls to some ``main'' \emph{proxy} contract are \emph{delegated} to sub-contracts. Although all these contracts are immutable, the proxy contract stores the addresses of the delegated sub-contracts in mutable variables. Thus, the proxy's functionality can be updated by changing these addresses.

\subsubsection*{The ``delegatecall'' Opcode}
The EVM facilitates contract-contract interaction in a myriad of ways, one of them relies on the \emph{delegatecall} opcode~\cite{buterin2015eip}. When this opcode is used during the execution of a contract $\mathcal{A}$, the execution is delegated to a contract $\mathcal{B}$ which is given as an argument to the opcode, where the latter contract's code is executed with the same environment variable scope as the former's, e.g., with the same \emph{sender} and \emph{value} variables.

\subsubsection*{The Proxy Design Pattern}
\label{section:proxyPattern}
While the code of a smart contract can not be altered after deployment, its state variables can change~\cite{dannen2017introducing,jezek2021ethereum}. For instance, an ERC-20 token may be implemented using a smart contract that holds a mapping between each holder's address and their balance of the token, with the balances liable to change due to user-user transfers.

The proxy pattern circumvents code immutability by relying on variable mutability. Concretely, this pattern splits logic into at least two contracts, where the function calls to the first ``proxy'' \emph{delegator} contract are forwarded to the second \emph{delegate} contract. The delegator stores the address of the delegate contract in a mutable variable, thereby allowing one to replace the delegate by simply changing this address and pointing it to a different contract. Changing the address of the delegate is allowed only by an address stored in the delegator's \emph{admin} variable. We provide a graphical depiction of this pattern in~\cref{fig:governance_proxy}.

\begin{figure}
    \centering
    \includegraphics[width=0.8\columnwidth]{governance_proxy}
    \caption{A graphical depiction of the \emph{Proxy Design Pattern}. This pattern allows to circumvent code immutability by relying on variable mutability. The owner of the ``main'' proxy contract can change the address of the implementation contract at any time.}
    \label{fig:governance_proxy}
\end{figure}
